Data Augmentation for Code Translation with Comparable Corpora and Multiple References

One major challenge of translating code between programming languages is that parallel training data is often limited. To overcome this challenge, we present two data augmentation techniques, one that builds comparable corpora (i.e., code pairs with similar functionality), and another that augments existing parallel data with multiple reference translations. Specifically, we build and analyze multiple types of comparable corpora, including programs generated from natural language documentation using a code generation model. Furthermore, to reduce overfitting to a single reference translation, we automatically generate additional translation references for available parallel data and filter the translations by unit tests, which increases variation in target translations. Experiments show that our data augmentation techniques significantly improve CodeT5 for translation between Java, Python, and C++ by an average of 7.5% Computational Accuracy (CA@1), which verifies the correctness of translations by execution. The code is available at https://github.com/Veronicium/CMTrans.

==> analysis.tex <==



==> init_exp.tex <==
\input{emnlp2023-latex/Tabels/cont_pretrain}
\input{emnlp2023-latex/Tabels/multi_ref}

\section{Initial Experiments}
We conduct initial experiments to answer the following research questions: 
\textbf{(RQ1)} How to our methods perform compared to baseline methods?
\textbf{(RQ2)} Will the model benefit from continuous pretraining?
\textbf{(RQ3)} Will the model benefit from multiple references in continuous pretraining, self-training, and finetuning?

\start{Datasets} We conduct Java-to-Python translation in the initial experiments. We use AVATAR-g4g as the finetuning dataset. For our method, we use AVATAR \citep{avatar} and xCodeEval \cite{xcodeeval} as the continuous pretraining dataset. 
For the self-training baseline \cite{transcoderST}, we use xCodeEval \cite{xcodeeval} to label self-training data.
We test all the methods on TransCoder-Eval \cite{transcoder} where human-designed test cases are provided.
We randomly sample up to 5 references for each source in xCodeEval and AVATAR. 
The statistics of the datasets after sampling are shown in Table \ref{tab:dataset}.

\start{Evaluation metrics} Following \citet{transcoder}, we use Computational Accuracy as the evaluation metric for the TransCoder dataset. CA@x, k=y means we generate y candidates by beam search,  select x candidates with the highest score, and count the percentage of test instances where at least one of these x candidates pass all the provided test cases.


\start{Comparison between methods} To answer \textbf{RQ1}, we show the comparison between our method and baselines in Table \ref{tab:main}. We can see that when combined with fine-tuning, both continuous pretraining and model-generated multiple references have a larger performance gain compared to the TransCoder-ST method \cite{transcoderST}.


\start{Continuous pretrain experiments} 
To answer \textbf{RQ2}, we show the experiments of continuous pretraining on different datasets in Table \ref{tab:cont}. 
We can see that training on the comparable corpora alone yields unsatisfactory performance, but when combined with fine-tuning on parallel data, we can obtain a large performance gain from continuous pretraining.
Keep increasing the size and diversity of continuous pretraining data further improves the performance.

\start{Training with multiple references} Table \ref{tab:multiref} and Table \ref{tab:selfmultiref} answer \textbf{RQ3} by presenting the comparison between training with multiple references in continuous pretraining and finetuning.
The results in Table \ref{tab:multiref} indicate that training with multiple references in both continuous pretraining and finetuning improves performance.
However, the gain from continuous pretraining and finetuning with multiple references cannot combine.
    

In Table \ref{tab:selfmultiref}, we can see that when we split training on self-labeled data and annotated data into two steps, using multiple references improves the performance.
However, similar to Table \ref{tab:multiref}, the performance gain from self-training and finetuning with multiple references cannot combine with the gain from continuous pretraining.


\input{emnlp2023-latex/Tabels/ST_multi_ref}

==> prev_intro.tex <==
\section{Introduction}
Software engineers are often required to migrate a codebase into another programming language.
Recently, language models pretrained on code \cite{codex,codegen,codebert} has shown a strong performance of neural code translation after finetuning on parallel data, where the program in source and target language have the same functionality, logic, and structure \cite{codexglue,transcoder,avatar} \yiqing{To do: put some examples in supplementary to show what is logic and structure}.
This provides the possibility of automatic codebase migration.
\dfried{Did any of these do code translation? Chen and Nijkamp did not. Maybe cite CodeT5 and PLBART instead?}

One major challenge of code translation is the parallel data is typically limited. For instance, the TransCoder \cite{transcoder} dataset only contains 466 Python-C++ pairs, and HumanEval-X \cite{codegeex} only contains 164. Constructing parallel data requires huge human effort and cannot be easily scaled up. 
To mitigate the data scarcity issue, previous work \citep{transcoderST} generates parallel data with self-training. It uses the unsupervised model to generate multiple translations for unlabeled functions and filters out incorrect translations with unit tests.
However, in self-training, it is likely that the majority of self-labeled data are easy examples, where the reference translation already has a high probability. This may lead to overfitting to easy examples, or even specific references \cite{ST3D,DataAugEasy}.
Furthermore, it is expensive to run unit tests to verify every generated translation. For instance, TransCoder-ST \cite{transcoderST} has verified translations for over 300K programs.
\dfried{This is pretty detailed but also a bit disconnected from our description of our approach. Can we make it clearer how our approach solves these issues, or save some of the detail for a related work section where we contrast with ours?}

Fortunately, we observe that code translation models can benefit from not only parallel data but comparable corpora, where the source and target programs have similar functionality and topic.
As shown in Fig. XX, after training on the comparable corpora for Java-Python translation, the perplexity is significantly reduced and converges to a lower value after finetuning.
\yiqing{To do}
It is also relatively easy to extract \cite{avatar,xcodeeval,codenet} or construct comparable corpora compared to parallel data since we do not require the source and target program to have the same logic and structure.
\dfried{Perplexity is a great thing to have in analysis, but reporting improved semantic match seems like a better thing to do in the introduction if possible}

In this paper, we present a data augmentation method for code translation that first train the model on comparable corpora before finetuning on parallel data.
Since existing datasets of comparable corpora mainly focus on the programming contests \cite{avatar,xcodeeval,codenet}, we further use code generation models to automatically construct comparable corpora for general domains.
Specifically, we extract functions in one language with docstrings, feed the docstring to code generation models trained in the other language and take the output program and the original function as a pair of training instances.
Since we do not need to verify the functionality of the generated programs, training on comparable corpora enjoys a more balanced distribution of hard and easy examples and better efficiency. 

To further mitigate overfitting to specific references, we augment the finetuning data with additional references generated by our model.
Specifically, we use our finetuned model to generate multiple candidates for each training instance, use automated test cases to filter out those with different behavior as the source code and select the most distinct subset with difflib.
Training with different translation references will provide the model with additional information about the equivalence of code snippets and hence avoid overfitting to one specific reference.
\dfried{Can we also count multiple references as a type of comparable corpora? Right now it's not clear whether the story is ``comparable corpora'' or ``comparable corpora + multiple references''. If the second, can we say something about why they go naturally together?}

\start{Contributions} (1) We train the code translation model on comparable corpora before finetuning and present a method of automatically constructing comparable corpora with generation models.
(2) We further avoid overfitting to specific references by finetuning with multiple references generated by the model itself.
(3) We will conduct experiments on multiple datasets and programming language pairs to demonstrate the utility of our methods.



==> to_do.tex <==
\section{Summary and future plans}
In summary, both continuous pretraining and finetuning/self-training with multiple model-generated references can improve code translation performance. 
However, these two techniques cannot well combine.

There are a few concerns to solve before submitting to EMNLP, especially when we are aiming at a long paper:
(1) \textbf{What is our idea to present?} Since the two techniques cannot combine well, I assume we cannot present both of them as our contributions. Also, I am not sure whether we need more interesting ideas to have better technical contributions. Our continuous pretraining experiments are done on existing datasets. Also, both AVATAR and xCodeEval also contain multiple references, and TransCoder-ST uses the model to generate multiple references and select one.

(2) \textbf{Can our methods be generalized to other settings?} After confirming the ideas, we still need to do experiments on multiple datasets on multiple language pairs.

I came up with some ideas to improve the technical contributions.
As extensions of continuous pretraining, we can: 
(1) Using code generation models (for source and target languages, each) to generate more comparable corpora.
(2) Using code with similar docstrings or descriptions as comparable corpora.
Both methods improve the scale and diversity of continuous pretraining data. Our current comparable corpora are mainly crawled from programming contests. With these methods, we can obtain comparable corpora with more diverse styles.

As extensions of training with multiple references, we can:
(1) Develop a loss function with multiple references. This can avoid having large weights on simple cases, where our model may generate more valid candidates as references.
(2) Use a re-ranking loss that ranks correct candidates before buggy ones. This utilizes buggy model-generated translations in addition to correct ones. This method can be viewed as using execution results as training signals in addition to similarity with the references, which also provides the model with more diverse information.

To try our methods on a wider range of datasets and language pairs, we can do the following experiments:

(1) Java $\leftrightarrow$ Python translation. Train on AVATAR-g4g and test on TransCoder-Eval, HumanEval-X (may need little modifications in training), and AVATAR-g4g (no execution-based evaluation).

(2) Java $\leftrightarrow$ C\# translation. Train and test on CodeXGLUE (no execution-based evaluation).

(3) Java $\leftrightarrow$ Python $\leftrightarrow$ C++ translation (low resource setting). Train on HumanEval-X and test on TransCoder-Eval.







